Semantic Communication based on Generative AI: A New Approach to Image Compression and Edge Optimization

As digital technologies advance, communication networks face challenges in handling the vast data generated by intelligent devices. Autonomous vehicles, smart sensors, and IoT systems necessitate new paradigms. This thesis addresses these challenges by integrating semantic communication and generative models for optimized image compression and edge network resource allocation. Unlike bit-centric systems, semantic communication prioritizes transmitting meaningful data specifically selected to convey the meaning rather than obtain a faithful representation of the original data. The communication infrastructure can benefit to significant improvements in bandwidth efficiency and latency reduction. Central to this work is the design of semantic-preserving image compression using Generative Adversarial Networks and Denoising Diffusion Probabilistic Models. These models compress images by encoding only semantically relevant features, allowing for high-quality reconstruction with minimal transmission. Additionally, a Goal-Oriented edge network optimization framework is introduced, leveraging the Information Bottleneck principle and stochastic optimization to dynamically allocate resources and enhance efficiency. By integrating semantic communication into edge networks, this approach balances computational efficiency and communication effectiveness, making it suitable for real-time applications. The thesis compares semantic-aware models with conventional image compression techniques using classical and semantic evaluation metrics. Results demonstrate the potential of combining generative AI and semantic communication to create more efficient semantic-goal-oriented communication networks that meet the demands of modern data-driven applications.

==> Include/Frontmatter/Titlepage_orig.tex <==
\begin{frontespizio}
% Remember: After editing this file, delete the cache and recompile
%---------------------Definizione font---------------------%
\Preambolo{\renewcommand{\fronttitlefont}{\fontsize{24}{24}\bfseries}}
%----------------------------------------------------------%
	% \frontinstitutionfont 	Neretto, 14/17 
	% \frontdivisionfont 		Tondo, 12/16 
	% \frontpretitlefont 		Maiuscoletto, 10/12
	% \fronttitlefont 		Neretto, 17/21 
	% \frontsubtitlefont 		Tondo, 12/14
	% \frontfixednamesfont 		Tondo, 12/14 
	% \frontnamesfont 		Neretto, 12/14 
	% \frontsmallfont 		Neretto, 9/11 
	% \frontfootfont	 	Neretto, 12/14 

	% \bfseries	Grassetto
	% \itshape	Corsivo
	% \scshape	Maiuscoletto
%----------------------------------------------------------%
\Margini{4cm}{3cm}{3cm}{3cm}				% Margini sinistro, in basso, destro e in alto
\Logo[4cm]{Figures/Logo/logo_sapienza_new.eps}
%\Universita{Roma}
\Istituzione{Sapienza University of Rome}
%\Facolta{Civil and Industrial Engineering}		% = 'Facolta di Ingegneria Civile ed Industriale'
\Divisione{Department name}		% = 'Facolta di Ingegneria Civile ed Industriale'
%\Dipartimento{Ingegneria Meccanica e Aerospaziale}	% = 'Dipartimento di Ingegneria Meccanica e Aerospaziale'
%\Corso[Master Degree]{Aeronautical Engineering}
\Scuola{PhD in XXXX Engineering}
\Titoletto{Thesis For The Degree Of Doctor Of Philosophy}
\Titolo{Generative Models for Semantic Communication: Exploring Semantic Compression and Modular Architectures}
%\Sottotitolo{}
\Punteggiatura{}					% Modifica la punteggiatura dopo 'Candidato', 'Realatore' ecc. (vuoto per togliere)
\NCandidato{Candidate}					% Sostituisce 'Candidato' con '...'
\Preambolo{\renewcommand{\frontsmallfont}[1]{\small}}
\Candidato[matricola]{Name}
%\Candidato{\small{1532252}}
\NRelatore{Thesis Advisor}{Relatori}			% Sostituisce 'Relatori' con 'Advisor' (permette anche di scrivere più relatori)
\Relatore{Prof. XXX XXX}
%\Correlatore{}
%\Rientro{1cm}						% Rientro di Relatore e Candidato
\Piede{Academic Year MMXIX-MMXXII (XXXV cycle)}					% A fondo pagina
\end{frontespizio}
\IfFileExists{\jobname-frn.pdf}{}{%
\immediate\write18{pdflatex \jobname-frn}}
